An Approximate Maximum Likelihood Time Synchronization Algorithm for Zero-padded OFDM in Channels with Impulsive Gaussian Noise

In wireless communication systems, Orthogonal Frequency-Division Multiplexing (OFDM) includes variants using either a cyclic prefix (CP) or a zero padding (ZP) as the guard interval to avoid inter-symbol interference. OFDM is ideally suited to deal with frequency-selective channels and additive white Gaussian noise (AWGN); however, its performance may be dramatically degraded in the presence of impulse noise. While the ZP variants of OFDM exhibit lower bit error rate (BER)and higher energy efficiency compared to their CP counterparts,they demand strict time synchronization, which is challenging in the absence of pilot and CP. Moreover, on the contrary to AWGN, impulse noise severely corrupts data. In this paper, a new low-complexity timing offset (TO) estimator for ZP-OFDM for practical impulsive-noise environments is proposed, where relies on the second-other statistics of the multipath fading channel and noise. Performance comparison with existing TO estimators demonstrates either a superior performance in terms of lock-in probability or a significantly lower complexity over a wide range of signal-to-noise ratio (SNR) for various practical scenarios.

==> Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido
%
%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
% ==== Computer Modern Sans Serif ====
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
%}
% =========================

% ==== Computer Modern Bright ====
% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
\DeclareFontShape{OT1}{cmbr}{m}{n}{%
  <-9>cmbr8
  <9-10>cmbr9
  <10-17>cmbr10
  <17->cmbr17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
  <-9>cmbrsl8
  <9-10>cmbrsl9
  <10-17>cmbrsl10
  <17->cmbrsl17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{it}{%
  <->ssub*cmbr/m/sl
}{}
\DeclareFontShape{OT1}{cmbr}{b}{n}{%
  <->ssub*cmbr/bx/n
}{}
\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
  <->cmbrbx10
}{}
% Part 2
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
}
% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareSymbolFont{sfletters}{U}{eur}{m}{n}\SetSymbolFont{sfletters}{bold}{U}{eur}{b}{n}%for Euler Greek
%\DeclareSymbolFont{sfletters}{FMS}{futm}{m}{n}\SetSymbolFont{sfletters}{bold}{FMS}{futm}{b}{n}%for Euler Greek

\DeclareMathSymbol{\sGamma}{\mathord}{sfletters}{0}
\DeclareMathSymbol{\sDelta}{\mathord}{sfletters}{1}
\DeclareMathSymbol{\sTheta}{\mathord}{sfletters}{2}
\DeclareMathSymbol{\sLambda}{\mathord}{sfletters}{3}
\DeclareMathSymbol{\sXi}{\mathord}{sfletters}{4}
\DeclareMathSymbol{\sPi}{\mathord}{sfletters}{5}
\DeclareMathSymbol{\sSigma}{\mathord}{sfletters}{6}
\DeclareMathSymbol{\sUpsilon}{\mathord}{sfletters}{7}
\DeclareMathSymbol{\sPhi}{\mathord}{sfletters}{8}
\DeclareMathSymbol{\sPsi}{\mathord}{sfletters}{9}
\DeclareMathSymbol{\sOmega}{\mathord}{sfletters}{10}
\DeclareMathSymbol{\salpha}{\mathord}{sfletters}{"0B}
\DeclareMathSymbol{\sbeta}{\mathord}{sfletters}{"0C}
\DeclareMathSymbol{\sgamma}{\mathord}{sfletters}{"0D}
\DeclareMathSymbol{\sdelta}{\mathord}{sfletters}{"0E}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfletters}{"0F}
\DeclareMathSymbol{\szeta}{\mathord}{sfletters}{"10}
\DeclareMathSymbol{\seta}{\mathord}{sfletters}{"11}
\DeclareMathSymbol{\stheta}{\mathord}{sfletters}{"12}
\DeclareMathSymbol{\siota}{\mathord}{sfletters}{"13}
\DeclareMathSymbol{\skappa}{\mathord}{sfletters}{"14}
\DeclareMathSymbol{\slambda}{\mathord}{sfletters}{"15}
\DeclareMathSymbol{\smu}{\mathord}{sfletters}{"16}
\DeclareMathSymbol{\snu}{\mathord}{sfletters}{"17}
\DeclareMathSymbol{\sxi}{\mathord}{sfletters}{"18}
\DeclareMathSymbol{\spi}{\mathord}{sfletters}{"19}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\ssigma}{\mathord}{sfletters}{"1B}
\DeclareMathSymbol{\stau}{\mathord}{sfletters}{"1C}
\DeclareMathSymbol{\supsilon}{\mathord}{sfletters}{"1D}
\DeclareMathSymbol{\sphi}{\mathord}{sfletters}{"1E}
\DeclareMathSymbol{\schi}{\mathord}{sfletters}{"1F}
\DeclareMathSymbol{\spsi}{\mathord}{sfletters}{"20}
\DeclareMathSymbol{\somega}{\mathord}{sfletters}{"21}
\DeclareMathSymbol{\svarepsilon}{\mathord}{sfletters}{"22}
\DeclareMathSymbol{\svartheta}{\mathord}{sfletters}{"23}
\DeclareMathSymbol{\svarpi}{\mathord}{sfletters}{"24}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}
\DeclareMathSymbol{\svarsigma}{\mathord}{sfletters}{"26}
\DeclareMathSymbol{\svarphi}{\mathord}{sfletters}{"27}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
%-------------------------
% Math symbol
%-------------------------
\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
\newcommand{\RV}[1]{\boldsymbol{\MakeLowercase{\msf{#1}}}}
\newcommand{\RM}[1]{\boldsymbol{\MakeUppercase{\msf{#1}}}}
\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}

\newcommand{\V}[1]{\boldsymbol{\MakeLowercase{#1}}}
\newcommand{\M}[1]{\boldsymbol{\MakeUppercase{#1}}}
\newcommand{\Set}[1]{\MakeUppercase{\mcal{#1}}}

